Mix-QSAM: Mixed-Precision Quantization of the Segment Anything Model

The Segment Anything Model (SAM) is a popular vision foundation model; however, its high computational and memory demands make deployment on resource-constrained devices challenging. While Post-Training Quantization (PTQ) is a practical approach for reducing computational overhead, existing PTQ methods rely on fixed bit-width quantization, leading to suboptimal accuracy and efficiency. To address this limitation, we propose Mix-QSAM, a mixed-precision PTQ framework for SAM. First, we introduce a layer-wise importance score, derived using Kullback-Leibler (KL) divergence, to quantify each layer's contribution to the model's output. Second, we introduce cross-layer synergy, a novel metric based on causal mutual information, to capture dependencies between adjacent layers. This ensures that highly interdependent layers maintain similar bit-widths, preventing abrupt precision mismatches that degrade feature propagation and numerical stability. Using these metrics, we formulate an Integer Quadratic Programming (IQP) problem to determine optimal bit-width allocation under model size and bit-operation constraints, assigning higher precision to critical layers while minimizing bit-width in less influential layers. Experimental results demonstrate that Mix-QSAM consistently outperforms existing PTQ methods on instance segmentation and object detection tasks, achieving up to 20% higher average precision under 6-bit and 4-bit mixed-precision settings, while maintaining computational efficiency.

==> sec/sup1.tex <==
\section{Supplementary Material}
\begin{figure*}[!t]
\centering
\setlength{\tabcolsep}{1pt} % slightly reduce tabular spacing
\begin{tabular}{ccccc}
  \includegraphics[width=2.7cm]{segmentation_fig/original/000000000785.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/FP/000000000785.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-S4/000000000785.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-L4/000000000785.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/Mix-QSAM4/000000000785.jpg} \\
  \includegraphics[width=2.7cm]{segmentation_fig/original/000000011149.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/FP/000000011149.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-S4/000000011149.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-L4/000000011149.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/Mix-QSAM4/000000011149.jpg} \\
  \includegraphics[width=2.7cm]{segmentation_fig/original/000000013291.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/FP/000000013291.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-S4/000000013291.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-L4/000000013291.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/Mix-QSAM4/000000013291.jpg} \\
  \includegraphics[width=2.7cm]{segmentation_fig/original/000000001532.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/FP/000000001532.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-S4/000000001532.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-L4/000000001532.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/Mix-QSAM4/000000001532.jpg} \\
  \includegraphics[width=2.7cm]{segmentation_fig/original/000000006040.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/FP/000000006040.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-S4/000000006040.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-L4/000000006040.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/Mix-QSAM4/000000006040.jpg} \\
  \includegraphics[width=2.7cm]{segmentation_fig/original/000000011760.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/FP/000000011760.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-S4/000000011760.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/PTQ4SAM-L4/000000011760.jpg} & \includegraphics[width=2.7cm]{segmentation_fig/Mix-QSAM4/000000011760.jpg} \\
  \makebox[2.7cm][c]{(a) Original} & 
  \makebox[2.7cm][c]{(b) Full Precision} & 
  \makebox[2.7cm][c]{(c) PTQ4SAM-S} & 
  \makebox[2.7cm][c]{(d) PTQ4SAM-L} & 
  \makebox[2.7cm][c]{(e) Mix-QSAM (Ours)} \\
\end{tabular}
\vspace{-2mm} % slightly reduce vertical spacing after caption
\caption{Qualitative comparison of instance segmentation on the COCO dataset using a 4-bit Segment Anything Model (SAM) with YOLOX bounding boxes as prompts. (a) Original images; (b) Full-precision SAM; (c) 4-bit PTQ4SAM-S without reconstruction; (d) 4-bit PTQ4SAM-L with reconstruction; (e) 4-bit Mix-QSAM (ours) without reconstruction.}
\label{fig:qualitative}
\end{figure*}

\subsection{Qualitative Results}
To evaluate the effectiveness of our method, we present qualitative instance segmentation results for 4-bit quantization of SAM on the COCO dataset, using YOLOX bounding boxes as prompts (Figure~\ref{fig:qualitative}). PTQ4SAM-S (without reconstruction) fails to segment objects accurately. Both PTQ4SAM-L (with reconstruction) and our Mix-QSAM preserve object integrity, produce clean boundaries, and retain fine-grained details. However, PTQ4SAM-L incurs significant computational overhead due to its blockwise reconstruction, which involves 20000 iterations. In contrast, Mix-QSAM delivers comparable visual quality without requiring reconstruction, making it a more efficient and practical solution for low-bit deployment.


==> supplementry.tex <==
% \documentclass[10pt, twocolumn, letterpaper]{article}
% \usepackage{cvpr}
\input{preamble}
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{makebox}

% \begin{document}
\title{Mix-QSAM: Mixed-Precision Quantization of the Segment Anything Model\\
Supplementary Material}
% \author{Navin Ranjan \hspace{0.75cm} Andreas Savakis\\
% Rochester Institute of Technology, Rochester, New York 14623, USA\\
% {\tt\small nr4325@rit.edu \hspace{0.5cm} andreas.savakis@rit.edu}}
% \twocolumn[{
% \maketitle

\date{}
\vspace{-1.0em}
\begin{center}
\renewcommand{\arraystretch}{0.5}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ccccc}
  \includegraphics[width=3.0cm]{segmentation_fig/original/000000000785.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/FP/000000000785.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-S4/000000000785.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-L4/000000000785.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/Mix-QSAM4/000000000785.jpg} \\
  \includegraphics[width=3.0cm]{segmentation_fig/original/000000011149.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/FP/000000011149.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-S4/000000011149.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-L4/000000011149.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/Mix-QSAM4/000000011149.jpg} \\
  \includegraphics[width=3.0cm]{segmentation_fig/original/000000013291.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/FP/000000013291.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-S4/000000013291.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-L4/000000013291.jpg}  & \includegraphics[width=3.0cm]{segmentation_fig/Mix-QSAM4/000000013291.jpg} \\
  \includegraphics[width=3.0cm]{segmentation_fig/original/000000001532.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/FP/000000001532.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-S4/000000001532.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-L4/000000001532.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/Mix-QSAM4/000000001532.jpg} \\
  \includegraphics[width=3.0cm]{segmentation_fig/original/000000006040.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/FP/000000006040.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-S4/000000006040.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-L4/000000006040.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/Mix-QSAM4/000000006040.jpg} \\
  \includegraphics[width=3.0cm]{segmentation_fig/original/000000011760.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/FP/000000011760.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-S4/000000011760.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/PTQ4SAM-L4/000000011760.jpg} & \includegraphics[width=3.0cm]{segmentation_fig/Mix-QSAM4/000000011760.jpg} \\
  \makebox[3.0cm][c]{(a) Original} & 
  \makebox[3.0cm][c]{(b) Full Precision} & 
  \makebox[3.0cm][c]{(c) PTQ4SAM-S} & 
  \makebox[3.0cm][c]{(d) PTQ4SAM-L} & 
  \makebox[3.0cm][c]{(e) Mix-QSAM (Ours)} \\
\end{tabular}
\captionof{figure}{Qualitative comparison of instance segmentation on the COCO dataset using a 4-bit Segment Anything Model (SAM) with YOLOX bounding boxes as prompts. (a) Original images; (b) Full-precision SAM; (c) 4-bit PTQ4SAM-S without reconstruction; (d) 4-bit PTQ4SAM-L with reconstruction; (e) 4-bit Mix-QSAM (ours) without reconstruction.}
\label{fig:qualitative}
\vspace{1em}
\end{center}

\section*{A. Qualitative Results}
To evaluate the effectiveness of our method, we present qualitative instance segmentation results for 4-bit quantization of SAM on the COCO dataset, using YOLOX bounding boxes as prompts (Figure~\ref{fig:qualitative}). PTQ4SAM-S (without reconstruction) fails to segment objects accurately. Both PTQ4SAM-L (with reconstruction) and our Mix-QSAM preserve object integrity, produce clean boundaries, and retain fine-grained details. However, PTQ4SAM-L incurs significant computational overhead due to its blockwise reconstruction, which involves 20000 iterations. In contrast, Mix-QSAM delivers comparable visual quality without requiring reconstruction, making it a more efficient and practical solution for low-bit deployment.
}]
% \end{document}

